Filaments and sheets of the warm-hot intergalactic medium

Filaments, forming in the context of cosmological structure formation, are not only supposed to host the majority of the baryons at low redshifts in the form of the WHIM, but also to supply forming galaxies at higher redshifts with a substantial amount of cold gas via cold steams. In order to get insight into the hydro- and thermodynamical characteristics of these structures, we performed a series of hydrodynamical simulations. Instead of analyzing extensive simulations of cosmological structure formation, we simulate certain well-defined structures and study the impact of different physical processes as well as of the scale dependencies. In this paper, we continue our work from Klar & M\"ucket (2010), and extend our simulations into three dimensions. Instead of a pancake structure, we now obtain a configuration consisting of well-defined sheets, filaments, and a gaseous halo. We use a set of simulations, parametrized by the length of the initial perturbation L, to obtain detailed information on the state of the gas and its evolution inside the filament. For L > 4 Mpc, we obtain filaments which are fully confined by an accretion shock. Additionally, they exhibit an isothermal core, which temperature is balanced by radiative cooling and heating due to the UV background. This indicates on a multiphase structure for the medium temperature WHIM. We obtain scaling relations for the main quantities of this core. In the vicinity of the halo, the filament's core can be attributed to the cold streams found in cosmological hydro-simulations. Thermal conduction can lead to a complete evaporation of the cold stream for L > 6 Mpc/h. This corresponds to halos more massive than M_halo = 10^13 M_Sun, and implies that star-formation in more massive galaxies can not be supplied by cold streams. For perturbations on scales L > 6 Mpc/h the filament does not longer exhibit a cold core.

==> Makefile <==
NAME = paper

all:
	latex $(NAME).tex && \
	bibtex $(NAME) && \
	sh bibfix.sh && \
	latex -interaction=nonstopmode $(NAME).tex && \
	latex -interaction=nonstopmode $(NAME).tex && \
	dvips $(NAME).dvi && \
	ps2pdf  -sPAPERSIZE=a4 $(NAME).ps

clean:
	rm -f $(NAME).aux $(NAME).blg $(NAME).dvi $(NAME).log $(NAME).pdf $(NAME).ps

